PADTHAI-MM: Principles-based Approach for Designing Trustworthy, Human-centered AI using MAST Methodology

Despite an extensive body of literature on trust in technology, designing trustworthy AI systems for high-stakes decision domains remains a significant challenge, further compounded by the lack of actionable design and evaluation tools. The Multisource AI Scorecard Table (MAST) was designed to bridge this gap by offering a systematic, tradecraft-centered approach to evaluating AI-enabled decision support systems. Expanding on MAST, we introduce an iterative design framework called \textit{Principles-based Approach for Designing Trustworthy, Human-centered AI using MAST Methodology} (PADTHAI-MM). We demonstrate this framework in our development of the Reporting Assistant for Defense and Intelligence Tasks (READIT), a research platform that leverages data visualizations and natural language processing-based text analysis, emulating an AI-enabled system supporting intelligence reporting work. To empirically assess the efficacy of MAST on trust in AI, we developed two distinct iterations of READIT for comparison: a High-MAST version, which incorporates AI contextual information and explanations, and a Low-MAST version, akin to a ``black box'' system. This iterative design process, guided by stakeholder feedback and contemporary AI architectures, culminated in a prototype that was evaluated through its use in an intelligence reporting task. We further discuss the potential benefits of employing the MAST-inspired design framework to address context-specific needs. We also explore the relationship between stakeholder evaluators' MAST ratings and three categories of information known to impact trust: \textit{process}, \textit{purpose}, and \textit{performance}. Overall, our study supports the practical benefits and theoretical validity for PADTHAI-MM as a viable method for designing trustable, context-specific AI systems.

==> archive/0abstract.tex <==
Designing AI systems that are deemed trustworthy remains a formidable challenge, compounded by the absence of actionable guidance despite an extensive body of literature on trust in technology. The Multisource AI Scorecard Table (MAST), a structured checklist rating system based on the U.S. Intelligence Community's Analytic Tradecraft Standards, seeks to bridge this gap by offering a systematic approach for both the design and evaluation of AI-enabled decision support systems. Expanding on the MAST framework, we introduce a comprehensive nine-step iterative design framework titled the \textit{Principled Approach for Designing Trustable Human-centered AI Systems using MAST Methodology} (PADTHAI-MM). This framework is exemplified through the development of the Reporting Assistant for Defense and Intelligence Tasks (READIT), an AI-enabled decision support system that leverages natural language processing for text analysis. To empirically assess the efficacy of MAST in enhancing trustworthiness, we developed two distinct iterations of READIT for comparison: a High-MAST version, which incorporates AI contextual information and explanations, and a Low-MAST version, akin to a ``black box'' system. This iterative design process was informed by participant feedback and leveraged state-of-the-art knowledge in AI, culminating in a refined prototype evaluated through its use in an intelligence reporting task. The findings from this evaluation highlight the potential benefits of employing the MAST framework on trust perceptions toward AI systems. Furthermore, our analysis delves into the relationship between participants' MAST ratings and three categories of information known to impact trust: \textit{process}, \textit{purpose}, and \textit{performance}. This investigation provides a robust theoretical framework that substantiates the utility of MAST in the context of trustable AI system design. Overall, our study shows the practical benefits and theoretical foundations for the proposed framework to advance the development of trustable AI-enabled decision support systems.

==> archive/1introduction.tex <==
\section{Introduction}

Recent strides in artificial intelligence (AI) have raised concerns \emily{about} trust and transparency given the potential impact that AI use may have in various decision settings. \mvm{Advanced AI technologies are being widely adopted across various domains, ranging from simple models like recommendation systems and chatbots to complex systems such as autonomous vehicles and large-scale language models.} However, the full appreciation of \mvm{these systems often requires an understanding of their underlying decision-making processes—an aspect that many people tend to overlook}~\citep{18, 10224086}. \emily{The demand for ``white-box'' models—algorithms with transparent logic and traceable decisions—has notably increased in high-stakes fields like healthcare and finance, where trust and transparency are paramount~\citep{8882211}.} \mvm{Despite this, the rapid expansion of AI applications has been predominantly fueled by black-box deep learning methods, which are known to perform excellently on complex tasks like face recognition and machine translation but are often criticized for their lack of transparency.}~\citep{rudin2019stop, duran2021afraid, london2019artificial}.

Efforts to improve the trustworthiness of black-box models without compromising their efficacy have led to the development of Explainable Artificial Intelligence (XAI)~\citep{Gunning_Aha_2019} methods. These strategies aim to overlay black-box models with post-hoc explanations, thereby rendering their decisions more comprehensible. Such explanations can range from representative predictions to IF-THEN rules or feature contribution analyses~\citep{1,2,3}. However, the effectiveness of these explanations in fostering trust is debatable, largely because they are typically designed from an engineer's perspective, which may not align with end-user expectations. Recent research supports this discrepancy, revealing \emily{that }while AI predictions can enhance decision-making, offering supplementary explanations on the prediction does not always impact performance~\citep{6}. 

Studies have consistently demonstrated a direct correlation between the transparency of an AI system and the trust people place in its decisions~ \citep{21,22,23}. A deficit in trust can lead to either naïve or avoidant interactions with AI systems, influenced by the perceived benefits and risks associated with system failures. Consequently, trust has emerged as a focal point of discussion alongside transparency and the groundbreaking progress of black-box models. Considering the recognized balance between transparency and performance in AI~\citep{laiHumanPredictionsExplanations2019}, trust is increasingly valued as a metric for algorithm selection within AI systems.

Theoretical frameworks based on empirical studies suggest that cultivating well-calibrated trust in AI requires considering multiple factors beyond simply providing explanations~\citep{chiou2023trusting,de2020towards}. Notably, trust in automation partly depends on an operator's understanding of the \textit{processes} (i.e., how it performs tasks), \textit{purpose} (i.e., why the system was developed), and \textit{performance} (i.e., how effectively it carries out those tasks) of the AI system~\citep{lee2004trust}. Recent work has indicated these three information categories can inform technology designers and evaluators on how operators trust a system and make informed decisions about its usage \citep{chancey2017trust}. Therefore, in addition to making AI \textit{processes} more explainable\emily{, as XAI approaches propose}, theoretical trust frameworks have long suggested that effectively designing for calibrated trust also requires operators' understanding of a system's intended function (i.e., \textit{purpose}) and reliability (i.e., \textit{performance})~\citep{8}.

However, previous literature has predominantly focused on the evaluation and design of black-box models for interpretability from technical perspectives ~\citep{10.1145/3236009} rather than evaluating these models specifically for trustworthiness. While algorithms providing high-quality explanations (e.g., LIME, SHAP, TabNet, and Anchors) have been used to evaluate model explainability (Mirzaei et al, 2023),  there is currently no formal method dedicated to evaluating these models from a trust perspective. Furthermore, some researchers have argued that excessive attention has been devoted to explanation interpretability, neglecting the interaction between black-box models and people (Shen, 2022). Consequently, this paper aims to extend beyond the focus on explanations and transparency by also considering the aspect of human-AI interaction that could influence trust and trustworthiness. 

General design guidelines for addressing human information needs associated with trust have been proffered from theoretical frameworks (e.g., \citealp{12, 17, lee2004trust}). However, these guidelines often require substantial human factors expertise to interpret abstract insights into actionable requirements at the implementation stage. Conversely, actionable guidelines for designing trustworthy AI systems tend to originate from industry standards or tradecraft, and the generalizability of these guidelines and connection to the empirical and theoretical research is often unclear. Among these is the Multisource AI Scorecard Table (MAST), which was developed by a group from the 2019 Public-Private Analytic Exchange program sponsored by the U.S. Department of Homeland Security's Office of Intelligence and Analysis, on behalf of the Office of the Director of National Intelligence (ODNI) \citep{blasch2021multisource}. MAST articulates nine criteria derived from analytic tradecraft standards specified in Intelligence Community Directive (ICD) 203 \citep{odniIntelligenceCommunityDirective2015} to help guide the design and assessment of AI system trustworthiness. These criteria include transparency qualities that are also commonly used in XAI approaches, such as Uncertainty (i.e., whether system outputs are displayed with information about possible levels of uncertainty) and Visualization (i.e., whether system outputs are displayed with graphics to aid user understanding). As a four-point Likert scale (0-3, with 0 representing ``poor'' and 3 ``excellent''), MAST is one of few tradecraft-derived scales for AI trustworthiness that have been validated against existing theoretically-derived and empirically-tested trust questionnaires \citep{chiou22}. For instance, MAST-oriented designs were shown to improve system operator perceptions of system trustworthiness, despite not guaranteeing improved overall system outcomes \citep{salehi2023evaluating}.

In this paper, we introduce a design framework called \textbf{PADTHAI-MM} (\textbf{P}rincipled \textbf{A}pproach for \textbf{D}esigning \textbf{T}rustable, \textbf{H}uman-centered \textbf{AI} systems using the \textbf{M}AST \textbf{M}ethodology) that integrates the MAST criteria with an iterative design process tailored for developing AI-enabled decision support systems (AI-DSS). Although PADTHAI-MM shares similar principles\emily{ to those} behind user-centered and work-centered design approaches for software systems (e.g., \citealp{Beyer_Holtzblatt_1999, Roth_Bisantz_Wang_Kim_Hettinger_2021}), PADTHAI-MM focuses more simply on how to incorporate organizational values and state of the art knowledge of technology capability with criteria for information quality that are widely adopted by the Intelligence Community. Whereas user-centered approaches tend to focus on operator goals and specifications that could improve technology adoption, and work-centered approaches tend to focus on reducing cognitive load\emily{—}both crucial for broader system design considerations\emily{—}PADTHAI-MM instead addresses the specific challenges that design teams may face when it comes to operationalizing state-of-the-art information processing tools with facets of information quality that can affect trust in AI-enabled decision support systems.

As a case study, we first demonstrate the efficacy of PADTHAI-MM in our development of a text summarization system called the \textbf{RE}porting \textbf{A}ssistant for \textbf{D}efense and \textbf{I}ntelligence \textbf{T}asks (READIT). To validate the impact of the MAST criteria as guiding design principles, we developed two versions of READIT, a ``High-MAST'' version designed to meet as many MAST criteria as possible, and a ``Low-MAST'' version that provided minimal functionalities necessary for task completion. We then involved study participants to compare the two versions, and to inform our iterative design process. To assess the theoretical validity of MAST as the foundational basis for PADTHAI-MM, we also used Principal Component Analysis (PCA) and feature categorization to investigate three types of information known to affect trust in supervised automated systems (purpose, process, performance; ~\citealp{lee2004trust}) and their associations with our designed READIT features and MAST rating goals. We first detail our design process and READIT case study below, before reporting the findings of our investigation. \\

==> archive/3framework.tex <==
\section{PADTHAI-MM: A MAST-inspired Design Framework}

The PADTHAI-MM design framework (\autoref{fig:3component}) integrates AI and data knowledge with current trust scholarship to develop trustable AI-DSSs according to the involved stakeholder needs. PADTHAI-MM comprises nine major steps and borrows from iterative design frameworks for product development~\citep{ulrich2008product}. We posit that each step contributes to improving system efficacy and alignment with organizational values. Design ideation and execution steps of PADTHAI-MM cover how to connect these qualities to corresponding AI features. 

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.9\textwidth]{figs/PADTHAI-MM-Overview.jpeg}
    \caption{PADTHAI-MM Design Framework}
    \label{fig:3component}
\end{figure}

A foundational step of PADTHAI-MM is to focus on the \emph{use case} or \emph{context}, i.e., identifying the needs and expectations of operators and other peripheral stakeholders where the AI-DSS will be deployed. This step addresses \textit{Customer Relevance}, a specified MAST criteria. After this ``opportunity recognition'' step, the design process moves to ``goal setting'' for system functionality and acceptable MAST ratings. This step is followed by ``iterative evaluation'' which involves design, test, and evaluation sub-processes until the previously set goals are satisfied.

Throughout the iterative evaluation step, design concepts or features attuned to the MAST criteria are generated to address stakeholder needs and expectations. These concepts or features must also be informed by the design team's knowledge of AI and data system concepts; including the principles, tools, and processes linked to the datasets that will be used by the AI-DSS. This requires the design team to identify how to fulfill system functionality and MAST rating goals simultaneously. For example, to satisfy the MAST \textit{Sourcing} criterion, we chose high-performing and interpretable AI algorithms and verified datasets to ensure the quality and credibility of underlying sources and methods. 

==> archive/4designprocess.tex <==
\subsection{Step 0: Opportunity Recognition}
The initial phase, Step 0, involves the identification of viable opportunities for implementing an AI-DSS. It is crucial at this stage to pinpoint and systematically engage with key stakeholders through interviews. This process aims to collect detailed insights regarding current workflows, highlighting specific challenges and inefficiencies within the existing system.

\subsubsection{Case study: READIT, a text summarization AI-DSS}
To illustrate the application of the PADTHAI-MM framework, we chose to develop a use case and platform within the natural language processing (NLP) domain, where MAST was initially situated~\citep{blasch2021multisource}, specifically \emily{focusing on }a tool that could support analysts in real-time intelligence reporting tasks. An example application would involve extracting and summarizing security-related information from social media platforms to evaluate public sentiment regarding the construction of a new U.S. consulate building in London.

\subsection{Step 1: Determine system functionality goals}
Step 1 involves establishing the objectives of the work system and evaluating which work processes could be enhanced or addressed by an AI-DSS. This includes determining which tasks the AI-DSS should undertake and identifying how the integration of AI-DSS might introduce, expand, enhance, or eliminate certain human work processes. Additional considerations include defining acceptable outputs for each process, system reliability expectations (e.g., permissible error rates within specified operational periods), and the potential implications of suboptimal outputs or system failures. Moreover, it is essential to consider ethical, regulatory, and legal constraints to delineate the system's operational boundaries. 

\subsubsection{Case study: Determining system functionality goals for READIT 1.0}
The initial READIT use case was to enable intelligence analysts to efficiently search and summarize extensive datasets of text-based social media content. This capability aimed to facilitate accurate assessments of public sentiment towards the construction of a new consulate building in London. We envisioned that the system would deliver two primary outputs: (1) a curated list of highly influential content, as determined by user reactions and reposts; and (2) an AI-generated extractive summary encapsulating the essence of a broad corpus of posts. This would allow users to search social media posts using keywords, which would then direct them to related content.

\subsection{Step 2: Determine MAST criteria goals} 
Step 2 involves assessing the significance of each MAST criterion and establishing rating goals. First, align the MAST criteria with the system objectives identified in Step 1, then evaluate the relative importance of each criterion. \emily{Multiple Decision Criteria Analysis (MCDA; \citealp{ferreiraMeasuringTradeoffsCriteria2013}) frameworks such as the ``House of Quality'' (\citealp{hauser66house}), can facilitate this evaluation process by providing a structured approach.} Understanding the relative importance between criteria is crucial for navigating potential design trade-offs in the feature generation and configuration phases.

This step also entails specifying desired ratings for each MAST criterion and an overall MAST score. Establishing target MAST ratings also allows for a comparison with our use case (\autoref{appendixA}), which can serve as a reference for developing relevant design concepts in subsequent steps. If the process involves redesigning an existing AI-DSS, evaluate the current system using MAST to pinpoint areas for improvement. 

\subsubsection{Case study: Determining MAST criteria goals for READIT 1.0}
To evaluate our design framework effectively, we designed two versions of READIT, a High-MAST version and a Low-MAST version. The High-MAST version was intended to secure the highest possible MAST ratings (i.e., scoring 3 or ``excellent'') by incorporating the necessary features and information transparency levels. For the Low-MAST version, we sought to meet the essential system functionality goals with minimal transparency design features, targeting a baseline MAST rating of 1 (``fair'') for each criterion. 

\subsection{Step 3. Conceptualize MAST-informed features}
After establishing the system functionality and MAST rating objectives, Step 3 is the ideation of AI system features or the identification of existing solutions to develop feature concepts. As features are conceptualized to address each candidate process identified in Step 1, their MAST ratings may also be estimated to determine their potential contributions to the MAST goals identified in Step 2. \emily{Teams engaged in developing critical, industrial-scale systems would benefit from documenting these preliminary ratings, to allow for a more rigorous evaluation of the potential variation range for each MAST criterion, and to possibly refine or reconsider the features to reduce the range. This would comprise an additional iterative step in the design process, although not explicitly depicted in \autoref{fig:3component}.} Features may address multiple candidate processes or multiple MAST criteria; thus, design teams should map how feature concepts address each of its target candidate processes and assign MAST rating estimates. Note that feature concepts generated at this step, including their interoperability, will be further refined in subsequent iterations before their inclusion in system-level configurations.

\subsubsection{Case study: Conceptualizing MAST-informed features for READIT 1.0}
For our case study, we focused on devising features that allow both experienced and naïve operators to quickly evaluate the underlying data context, algorithmic performance, and algorithmic processes used by the AI-DSS to generate its outputs. A research team member (co-author A.P.) initially drafted the feature descriptions and proposed a MAST rating for each one. \emily{Subsequently, our team of computer scientists, industrial engineers, and human systems engineers engaged in a series of discussions and collectively reviewed and reached a consensus on the feature descriptions and their corresponding MAST ratings. }

Below, we summarize the feature concepts in High-MAST READIT 1.0 (\autoref{fig:MAST_rh}) within each of the nine MAST criteria. For comparison, feature concepts for Low-MAST READIT 1.0 (\autoref{fig:MAST_rl}) are also presented. Detailed definitions of each MAST item and the corresponding features in READIT High-MAST and Low-MAST versions are provided in \autoref{appendixA}.

\begin{enumerate}
\item \textbf{Sourcing} emphasizes the quality and credibility of the system's underlying sources, data, and methodologies. A \textit{Raw Content} feature that showcases raw datasets alongside their summaries (\autoref{subfig:rh1}) addresses this criterion. The \textit{Diagnostics}, \textit{Data Sheet}, and \textit{Date Range} features (\autoref{subfig:rh3}) offer essential information about the training data, its cleaning and extraction process, as well as metadata concerning the source data. The \textit{Diagnostics} feature displays the original data source locations, the number of original poster accounts, and the number of pieces of content or posts with uncertainty factors. \textit{Comparison Summary} feature (\autoref{subfig:rh2}) enables users to distinguish content from larger organizations, such as news media firms, from that of individual accounts.

\item \textbf{Uncertainty} addresses the impact of uncertainty factors on key analytic judgments. The \textit{Diagnostics} feature provides diagnostic information about uncertainties in the underlying content (e.g., misspellings, foreign characters or emojis, excessive punctuation, and fabricated content) and accentuates these factors in the raw content. An \textit{Alternative Summary needed} alert appears in the left window(\autoref{subfig:rh4}) if data integrity issues are likely to affect the final summary.

\item \textbf{Distinguishing} gauges the system's capability to differentiate underlying intelligence from its assumptions and judgments. \emily{For example, discerning which information is derived from the AI-DSS and which might originate from corrupted sources helps distinguish between system inputs and outputs to facilitate decision-making.} Utilizing off-the-shelf algorithms, the \textit{Diagnostics} feature infers the likelihood of content being human- or machine-generated disinformation, drawing analysts' attention to the content's quality or intent behind the information posted, rather than accepting the results uncritically.

\item \textbf{Analysis of Alternatives}  concerns the system's capacity to assess various decision options and provide alternative outcomes when data uncertainty exceeds a predefined threshold. The \textit{Alternative Summary needed} feature alerts users when the uncertainty factors necessitate an alternative summary. For instance, should the content contain numerous misspellings or predominantly consist of fake news, this feature would prompt the user to generate a new summary using an alternative set of keywords. Upon activation of this alert, uncertainty factors are \emily{also} highlighted within the \textit{Raw content} feature  (\autoref{subfig:rh4}).

\item \textbf{Customer Relevance} addresses the implications of system outputs and the system's ability to support users' needs and expectations. READIT 1.0 targets a college-educated U.S. demographic, especially working intelligence analysts with varied experience levels. In conjunction with the data and AI models anticipated to be available, we designed informative, concise text summaries for the \textit{Most Influential Content} and \textit{Extractive Summary} features (\autoref{subfig:rh1}). The \textit{Content Shown} feature (\autoref{subfig:rh3}) indicates the number of social media posts included in the summaries. The \textit{Diagnostics} and \textit{Word Cloud} features provide insights into the content creators (e.g., how long it has been active, how often content is created by the account, etc.) and the prevalence of content, respectively. 

\item \textbf{Logical Argumentation} pertains to the system's application of clear and logical reasoning in elucidating the AI's information generation process. Considering the potential impact of social media on intelligence task outcomes, search results in the \textit{Summary} and \textit{Raw Content} features are ordered based on the number of followers. \textit{Extractive Summaries} are ranked based on their significance scores (i.e., the occurrence frequency of the search terms within each content piece), designed to align with the user's manual content review process.

\item \textbf{Consistency} emphasizes the system's capability to explain the relevance of, or changes in, analytic judgments over time. To meet this criterion, one approach is to facilitate comparisons of AI recommendations (or operator decisions) within or across working sessions. The \textit{Comparison Summary} feature provides statistics for two selected summaries to compare and contrast the results. Additionally, operators have the option to generate a comparison summary with custom keywords to analyze how new findings align\emily{ with} or differ from prior results (top of \autoref{subfig:rh2}).

\item \textbf{Accuracy} \emily{pertains to the precision of a system's judgments and assessments, and the clarity with which these judgments are presented; it aims to minimize ambiguity around the likelihood, timing, and nature of decision parameters.} The \textit{Date Range} and \textit{Diagnostics} features show the date, time, and location of each content item, alongside a comprehensive metadata report. These features allow operators to accurately assess content relevance and quality during the analysis.

\item \textbf{Visualization} describes a system's integration of effective visual data displays where appropriate, such as graphical representations of the raw data or the outcomes of statistical analyses. The \textit{Visualizations} feature (bottom of \autoref{subfig:rh2}) incorporates various graphical representations, including word frequency bar charts, histograms of content distribution over time, word clouds, and webs of original poster networks, among others. These visualizations are clearly labeled and designed for straightforward interpretation without the need for additional references. 
\end{enumerate} 

\subsection{Step 4. Generate MAST-informed system mockups}
Step 4 is dedicated to creating system-level mockups by initially assessing the compatibility of each feature concept identified in Step 3.  The assessment criteria should include: (1) the feasibility of displaying features simultaneously within the constraints of interface space and human perceptual limitations \citep{Fitts_1954}; (2) the potential impact of feature workflows and interaction modalities on performance, especially concerning process or information redundancies, and; (3) the likelihood of feature concepts confusing users when gauging system trustworthiness, usability, or algorithmic performance. 

Upon assessing feature compatibility, system mockups are generated with a configuration of features that encompasses the candidate processes outlined in Step 1. The goal is to generate a variety of audiovisual or storyboard-like mockups rather than functional prototypes. These mockups should communicate user interactions with the system detailing required inputs and anticipated outputs. They facilitate swift assessment by stakeholders, allowing for a comparative analysis of how each configuration aligns with system functionality and other objectives established in Steps 1 and 2.

\subsubsection{Case study: Generating MAST-informed system mockups for READIT}
Leveraging our set of MAST-informed feature concepts, we created system mockups of High-MAST and Low-MAST versions, as depicted in \autoref{fig:MAST_rh} and \autoref{fig:MAST_rl}, respectively. The High-MAST mockup comprises three windows: (1) the \textit{Main Page} (\autoref{subfig:rh1}), featuring a keyword search bar alongside summaries and source texts; (2) the \textit{Tools} window (\autoref{subfig:rh2}), \emily{accessible via a button on the main page, offering advanced search options and content visualizations;} and (3) the \textit{Options} (\autoref{subfig:rh3}) window, presenting data specifics such as date range, dataset size, and content flagged for false information, special characters, or misspellings. Additionally, the High-MAST version incorporates an alert feature that prompts users to consider alternative summaries when search results surpass a predefined threshold. In contrast, the Low-MAST mockup consists of a single window comprising only essential features necessary for task completion: (1) a keyword search bar; and (2) a display area for search results showcasing the most influential content and their extractive summaries.

\begin{figure}[!htbp]
    \centering
    \begin{subfigure}{0.9\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/MAST-RH-1.jpg} 
        \caption{Main page of High-MAST READIT 1.0}
        \label{subfig:rh1}
    \end{subfigure} 
    \begin{subfigure}{0.9\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/MAST-RH-2.jpg}
        \caption{\textit{Tools} window}
        \label{subfig:rh2}
    \end{subfigure} 
\end{figure}

\begin{figure}[!htbp]
    \ContinuedFloat
    \centering
    \begin{subfigure}{0.9\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/MAST-RH-3.jpg}
        \caption{\textit{Options} windows}
        \label{subfig:rh3}
    \end{subfigure}
    \begin{subfigure}{0.9\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/MAST-RH-4.jpg}
        \caption{Alert in High-MAST READIT 1.0}
        \label{subfig:rh4}
    \end{subfigure}
    \caption{\nk{Demonstration of the READIT 1.0 platform under high-MAST conditions. (a) Main page when searching for a keyword, (b) two options of \textit{Tools} window, (c) four \textit{Options} windows, and (d) an example alert. Blue boxes highlight the features fulfilling the corresponding MAST criteria.}}
    \label{fig:MAST_rh}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{figs/MAST-RL.jpg}
    \caption{\nk{Example search result of Low-MAST READIT 1.0 demonstrating the platform's functionality when fulfilling minimum MAST criteria conditions, serving as a counterpart to Figure 2.}}
    \label{fig:MAST_rl}
\end{figure}

\subsection{Step 5. Determine MAST ratings for AI system mockups}
Following the generation of several system mockups as design alternatives (i.e., until the range of implementable solutions reaches saturation), \emily{Step 5 involves gathering stakeholder feedback}, including MAST criteria ratings, perceptions of usability, and functionality. This process might necessitate the development of supplementary informational materials (e.g., audio-visual aids) to elucidate the execution of processes identified in Step 1 within each mockup, thereby establishing a foundational understanding of the system's functionality as delineated by the incorporated features. It is advisable to enlist stakeholders (e.g., operators and subject matter experts) as evaluative study participants, assigning them randomly to review different system alternatives and providing them with relevant informational materials. Participants are then expected to furnish their MAST ratings of the system mockup, and complete questionnaires about perceived usability and other assessment tools depending on the goals and processes identified in Step 1. \emily{Additionally, conducting interviews and focus groups can yield valuable feedback, potentially uncovering unforeseen trade-offs that could inform the decision to either further iterate the design or move towards finalization. }

\subsubsection{Case study: Determining MAST ratings for READIT system mockups}
To determine MAST ratings for READIT 1.0 system mockups, we orchestrated an experimental study as shown in \autoref{fig:flowchart}.

\begin{enumerate}
    \item \textbf{Procedure.} 43 Participants were recruited through Prolific (www.prolific.com), where 26 tested Low-MAST and 17 tested High-MAST READIT. To access the study, participants were directed to a Qualtrics survey link \citep{Qualtrics}. The first page asked participants to provide their Prolific IDs and an IRB-approved informed consent was administered. Participants were then directed to a task description page that asked them to imagine a fictional scenario in which they were U.S. intelligence analysts, \emily{whose} main task was to monitor the news for any ongoing threats to public safety. They were told that to aid them in this task, they would be using an AI-enabled decision support system (i.e., READIT), a technological aid meant to supplement their own skills. Participants were informed that they would not be able to interact with READIT, but that they would be presented with an audio-visual walk-through and description of the tool's interface and features. To check for engagement and comprehension, participants were asked to complete a short pass/fail quiz relating to the content of the task and READIT descriptions. Participants who did not pass were removed from the remainder of the study. Lastly, participants were asked to complete an evaluation of the system using MAST and respond to questionnaires with items measuring trust, task engagement, and usability.

    \begin{figure}[!h]
    \centering
    \includegraphics[scale=0.5]{figs/flowchart.pdf}
    \caption{Evaluation Study Procedure for READIT 1.0. \textit{N} = 43 participants were recruited from Prolific, with \textit{n} = 23 participants randomly assigned to the High-MAST condition, and \textit{n} = 17 randomly assigned to the Low-MAST condition before receiving task instructions.}
    \label{fig:flowchart}
    \end{figure}

    \item \textbf{Independent Variable: System design.} Mockups of the High-MAST and Low-MAST versions of READIT 1.0 were administered as a randomly assigned between-subjects condition. Detailed descriptions of the features and descriptions for each version can be found in the preceding sections, and are illustrated in \autoref{fig:MAST_rh} and \autoref{fig:MAST_rl}.
    
    \item \textbf{Dependent variables: MAST criteria and trust perceptions.} The nine MAST criteria were administered using an adaptation of the \cite{blasch2021multisource} four-point MAST scale, with ``1'' representing ``poor'' and ``4'' representing ``excellent''. After initial pilot testing, our team decided to rephrase each MAST criterion as a question accompanied by its relevant feature description, as shown in \autoref{appendixB}. 
    % Appendix D and Appendix E lists MAST criteria and feature descriptions for \emph{READIT 1.0}. 
    The MAST-total score was calculated by adding these 9 criteria with a min - max range of 9 - 36. 
    % Participant perception of risk and benefit was measured by two single items \citep{weber2002domain}. 
    We also administered two well-known questionnaires used to assess people's trust in automation, with 12 items \citep{jian2000foundations} assessing general trust and 15 items \citep{chancey2017trust} assessing three types of information known to affect trust in automation: performance, process, and purpose. Each item was rated on a seven-point Likert scale, with ``7'' indicating ``extremely agree'' and ``1'' indicating ``extremely disagree''. We calculated the average rating, including the average from each subcategory in \cite{chancey2017trust}, to form the trust perception scores.
    % To measure credibility, we adopted a 3-item survey \citep{appelman2016measuring}. 
    % For more information regarding these variables refer to Appendix D which presents the scale, sample item, number of items for each variable, and Cronbach’s alpha.
    
    \item \textbf{Control Variables: Engagement, and usability.} To avoid common confounding factors that could affect the MAST and trust ratings for READIT, we also measured perceptions of READIT usability and task engagement. \emily{Usability was measured with a 10-item questionnaire \citep{brooke2020sus} and engagement with a 17-item questionnaire \citep{schaufeli2002measurement}. }

    \item \textbf{Results.} Study results showed that the High-MAST group compared to the Low-MAST group was significantly different (descriptively higher) on the MAST ratings (on 8/9 criteria, except \textit{Customer Relevance}) and also significantly different (descriptively higher) on the trust responses. 
% and lower perceived risk scores than the Low-MAST group. Also, benefit and credibility ratings were also higher for the High-MAST group than for the Low-MAST group. 
In addition, usability and engagement were not significantly different between High-MAST and Low-MAST groups. 

\end{enumerate}

\subsection{Step 6. Iterating feature and mockup designs}
Step 6 focuses on refining the initial mockups into working prototypes after analyzing stakeholder responses (Step 5) of the initial mockups and alternatives generated in Step 4. The results of the analysis should be compared to the system and MAST criteria goals determined in Steps 1 and 2, respectively. These should also be interpreted in light of the system features and MAST criteria mapping in Step 3. In some cases, as in our READIT case study, Step 6 may result in the AI-DSS use case being reconceptualized to better suit stakeholder needs identified in Step 0 of the PADTHAI-MM framework. 

Depending on the analysis results, the design team (ideally including AI engineers, human systems engineers, and task domain experts) should recommend which system alternatives are ready for prototyping, need further design iterations, or should be discarded. Feature concepts and system mockups in need of further design iterations should roughly follow the procedure outlined in Steps 3 and 4. Step 6 ensures that expectations about the system's qualities remain within reasonable boundaries that are acceptable to the team. 

\subsubsection{Case study: Iterating feature and mockup designs for READIT}
\emily{After analyzing the study data, our team revisited the READIT 1.0 system mockups to discuss its use case and the feasibility of implementation in light of our available resources (e.g., datasets, servers, project personnel, timeline, and state-of-the-art models with similar functions).} We assessed READIT 1.0 from three perspectives: feasibility, task performance ability, and usability of the Low-MAST and High-MAST versions. We concluded that the initial mockup presented to participants was not implementable as a functional or credible working prototype for actual intelligence analyst use cases. Consequently, based on numerous project team discussions and feedback from pilot participants and project stakeholders, we redesigned the use case and system as \textbf{READIT 2.0}.
% We thus designed READIT 2.0 for practical use and human-AI interaction studies. 

\paragraph{READIT 2.0 Use Case.} One of the main constraints was that the original use case (i.e., gauging public sentiment from social media) could not be tested with an appropriate dataset to support the analysis and data visualization features we envisioned, and generating our own datasets would have gone beyond the scope of our project. Therefore, we adopted a new but similar use case for READIT 2.0, based on a corresponding available dataset from the VAST Challenge 2011 MC3 \citep{IEEEVAST2011MC3}: Investigation into Terrorist Activity. In this task, participants play the role of intelligence analysts searching for information related to potential terrorist activity among thousands of given news reports. Consultation with project stakeholders confirmed that this revised task sufficiently aligned with real-world situations encountered by analysts. 

\paragraph{READIT 2.0 Features and Mockups.} We again developed Low-MAST and High-MAST versions for READIT 2.0 to further demonstrate the utility of PADTHAI-MM, illustrated in \autoref{fig:readit_new_comparison}. Instead of the extractive summaries that select and rearrange existing content from original text sources, we designed READIT 2.0 to present abstractive summaries that generate new content to describe news data. For the High-MAST version (\autoref{subfig:newrh}), we designed three data visualization features: \textit{Topic Clusters}, a \textit{Topic Similarity Matrix}, and a \textit{Topic Timeline}. A feature was also designed to provide users with \textit{raw content} when operators click on the summary box, as well as a list of all topics along with checkboxes to narrow down the range of summary results. The Low-MAST version (\autoref{subfig:newrl}) does not provide \textit{Topic Clusters} nor additional information buttons for each section, but maintains basic functionality for operators to complete the given task within a reasonable time frame. 

After designing the READIT 2.0 mockups, our team assessed the two designs to ensure that the MAST rating goals would be met (``excellent'' for High-MAST, ``fair'' for Low-MAST). \autoref{tab:readit_mast} presents the results of this process, in which each rating represents the outcome of a group discussion and is presented as a binary rating (yes/no) to support efficient decision-making and minimize ambiguity. To fulfill MAST criteria goals, additional features were added to the High-MAST version, including information about the platform and technologies used, as well as a visualization of the topics from the raw documents. To further streamline the Low-MAST version, certain components were simplified, resulting in some functions being omitted. For example, the Low-MAST \textit{Topic Similarity matrix} lacked a selection feature, the \textit{Topic Timeline} lacked a timeline selection option, and the \textit{Documents \& Summaries} did not visualize the documents (presenting only a summary).  \autoref{appendixB} presents the detailed features in READIT 2.0 matching each MAST criterion. 

\begin{figure}[htbp]
    \centering
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/new-RH-main.jpg}
        \caption{High-MAST READIT 2.0}
        \label{subfig:newrh}
    \end{subfigure} \hfill
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/new-RL-main.jpg}
        \caption{Low-MAST READIT 2.0}
        \label{subfig:newrl}
    \end{subfigure} 
    \caption{(a) Main page of High-MAST and (b) Low-MAST of READIT 2.0. Compared with the Low-MAST, High-MAST has more interactive features (\textit{Topic Clusters}, information buttons, dropdown option in \textit{Topic Similarity}, etc.) and information (\textit{Documents} and \textit{About} tab) to demonstrate MAST criterion.}
    \label{fig:readit_new_comparison}
\end{figure}

\begin{table}[h]
\tiny
\centering
    \begin{tabular}{p{0.12\linewidth}|c|c|c|c|c|c|c|c}
      \toprule % <-- Toprule here
      Interface Items & \textbf{\makecell{Data\\Preprocess}} & \textbf{\makecell{Documents\\Tab}} & \textbf{\makecell{About\\Tab}} & \textbf{\makecell{Documents\\ \& Summaries}} & \textbf{\makecell{Topic\\Clusters}} & \textbf{\makecell{Topic\\Similarity\\Matrix}} & \textbf{\makecell{Topic\\Filtering}} & \textbf{\makecell{Topic\\Timeline}} \\ 
      \midrule % <-- Midrule here
      \textbf{Sourcing} & \checkmark \bluecheckmark & \checkmark & \checkmark & \checkmark & \checkmark & & & \checkmark \\
      \midrule % <-- Midrule here
      \textbf{Uncertainty} & & & \checkmark & & & \checkmark  &  \\
      \midrule % <-- Midrule here
      \textbf{Distinguishing} & & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark  & \checkmark \\    
      \midrule % <-- Midrule here
      \textbf{Analysis of Alternatives} & & & \checkmark & & \checkmark & \checkmark & \checkmark & \\
      
      \midrule % <-- Midrule here
      \textbf{Customer Relevance} & & & & \checkmark & \checkmark & \checkmark \bluecheckmark & \checkmark \bluecheckmark & \checkmark \bluecheckmark\\                             
      \midrule % <-- Midrule here
      \textbf{Logic} & & & \checkmark & \checkmark \bluecheckmark & \checkmark & \checkmark \bluecheckmark & \checkmark & \checkmark\\
      
      \midrule % <-- Midrule here
      \textbf{Change} & & \checkmark & \checkmark & & & \checkmark &  \\
      \midrule % <-- Midrule here
      \textbf{Accuracy} & & & \checkmark & & \checkmark & & & \\
      \midrule % <-- Midrule here
      \textbf{Visualization} & \checkmark \bluecheckmark & & & \checkmark & \checkmark & \checkmark \bluecheckmark & \checkmark & \checkmark \\         
    \bottomrule % <-- Bottomrule here
    \end{tabular}
    \vspace{20pt} \caption{MAST criteria in READIT 2.0. Red checkmarks and blue checkmarks denote High-MAST and Low-MAST versions respectively. Each row represents a specific MAST criterion and the columns show details for the front-end interface, which include various functions presented by the AI system, such as descriptive and calculated details, alerts, pop-up boxes, and buttons.}
  \label{tab:readit_mast}
  % \end{center}
\end{table}

\subsection{Step 7. Generating MAST-informed working prototypes.}
Step 7 develops the system design identified at the end of Step 6 into a working prototype. At this step, minor modifications approved by the design team should still be expected as designs are translated into working programs.

\subsubsection{Case study: Generating MAST-informed working prototypes for READIT}
READIT 2.0 was prototyped as a JavaScript-based client to facilitate interactivity between participants and the AI-DSS. The server was developed using Python 3 and Flask library and hosted on the Google Cloud Platform. To enhance operators' ability to explore the dataset, READIT 2.0 included various data visualizations. These visualizations were implemented using React, a well-known JavaScript library used for creating personalized and interactive data visualizations.  

We designed the abstractive summary generation feature of READIT 2.0 using PEGASUS \citep{zhang2020pegasus}, a state-of-the-art deep learning-based text summarization algorithm. The model uses the transformer encoder-decoder structure. Input text is encoded as a numerical context vector, which is then decoded to generate the abstractive summaries. The model is pre-trained to choose and mask important sentences and then recover them, a process called Gap Sentence Generation. We used the cnn\_dailymail dataset for pre-training PEGASUS. Both High-MAST and Low-MAST working prototypes of READIT 2.0 included a functional front-end interface that allowed access to various natural language processing and visualization features executed in the back-end. The code is available here: https://github.com/nayoungkim94/PADTHAI-MM.

\subsection{Step 8. Determining MAST ratings for working prototypes}
In alignment with Step 5,  it is essential to engage potential system users and stakeholders for the hands-on evaluation of the working prototypes developed in Step 7. This involves designing a task scenario that mirrors the operational environment in which the system will be deployed. In addition to soliciting system evaluations through questionnaires and interviews as outlined in Step 5, it is also crucial to measure participants' performance in decision-making tasks against the system functionality goals and metrics established in Step 1.

\subsubsection{Case study: Determining MAST ratings for READIT working prototypes}
We recruited intelligence analysts (IAs) primarily from the U.S. Department of Homeland Security (DHS), but also from other agencies, to operate and test READIT 2.0. The resulting 23 respondents were all analysts from the DHS. Analysts were randomly assigned to either a High-MAST or Low-MAST version and tasked with using READIT in a hypothetical scenario aimed at identifying potential \nk{patterns} of a terrorist attack. Afterward, participants were asked to assign MAST criteria ratings and complete the trust questionnaires developed by \cite{jian2000foundations} and \cite{chancey2017trust}, which were previously used to evaluate READIT 1.0. 

Our findings show the High-MAST group exhibited descriptively higher ratings across 8 of the 9 MAST criteria, with the exception of \textit{Customer Relevance}, and displayed significantly higher trust ratings in the ``purpose'' dimension \citep{chancey2017trust} compared to the Low-MAST group.
% , and lower perceived risk scores than the Low-MAST group. 
% Also, benefit and credibility ratings were also higher for the High-MAST group than for the Low-MAST group. 
Concerning usability and engagement, no significant differences were observed between the groups. Notably, the High-MAST group required an average of 10 additional minutes to complete the task relative to the Low-MAST group. For a more detailed report, the complete study is documented in~\cite{salehi2023evaluating}.


\subsection{Step 9. Determining if further design iterations are needed}
Upon evaluating the working prototypes in Step 8, the design team should conduct statistical analyses of questionnaire responses and performance metrics, comparing these findings against the system functionality and MAST rating goals established in Steps 1 and 2. Should any of the prototypes meet the predefined performance and MAST rating benchmarks, the design team and stakeholders must decide which prototype(s) warrant advancement toward an implementation \emily{phase}. Conversely, if none of the prototypes satisfy the performance or MAST criteria goals, the design process should recommence from Step 7. If it is collectively determined that achieving the set performance and MAST criteria objectives is unfeasible, the process should then revert to Step 1 or 2.

\subsubsection{Case study: Determining further iteration design needs for READIT 2.0}
Following the examination of participant feedback on READIT 2.0, our design team concluded that the system successfully fulfilled our specified functionality and MAST criteria objectives. Given that the primary aim of this project was to facilitate research, we decided against pursuing further design iterations.



==> archive/5evaluation.tex <==
\section{Theoretical Evaluation of MAST-Inspired Design Framework}
This section outlines the theoretical validation of our proposed design framework, focusing on the interplay between MAST-inspired design features of READIT 2.0 and participant responses to the~\cite{chancey2017trust} trust questionnaire, with items grouped according to the trust information categories of process, purpose, and performance~\citep{lee2004trust}.  

\subsection{Results}
Leveraging responses to the MAST questionnaire (as detailed in Step 9), we established a correlation between the MAST criteria and the specific features implemented in READIT 2.0. This correlation was quantitatively assessed through a linear transformation, which involved the computation of an inner product between the matrix of MAST evaluations and the matrix representing the mapping of MAST criteria to READIT 2.0 features.

\subsection{Method: Principal Component Regression}
Our team (EC, MM, NK, YB, SB, PS) categorized MAST criteria into three trust-related information types: \textit{process}, \textit{purpose}, and \textit{performance} (PPPs). \emily{We finalized the categorization through voting, discussion, and consensus.} These three categories derive from scholarship on interpersonal trust in organizations (i.e., ability, integrity, benevolence respectively) in ~\cite{mayer1995integrative} and have been connected to empirical studies in a literature review on trust in automation ~\citep{lee2004trust}. 

% Specifically, \textit{Performance} refers to the system's functionality and its effectiveness in fulfilling the operator's goals. \textit{Process} describes the information related to the system's underlying algorithms and whether the algorithms are capable of achieving the operator's goals. \textit{Purpose} denotes the intended use of the system as defined by the designers, reflecting its alignment with the operator's goals. 

% For example, performance should exhibit the user's outputs clearly, process should be transparent and explainable, and purpose be related to a high-level description of the whole system.

Given the influence of MAST criteria on the design features of READIT 2.0 (as detailed in \autoref{tab:readit_mast}), we conducted a principal component analysis (PCA) to show the relationships between key features and the types of trust-related information (PPPs) distinguished in~\cite{chancey2017trust}. PCA is a dimensionality reduction technique, enabling the transformation of high-dimensional data sets into more manageable, lower-dimensional representations. This is achieved by identifying patterns in relationships among variables and capturing the maximum variance within the data. We set a threshold of 0.3 for the absolute values of factor loadings, with the aim of selecting principal components that account for at least 80\% of the data's cumulative variance with the initial $k$ principal components. Consequently, features exceeding this threshold were considered significant contributors to the PPPs.

For the subsequent analysis, we used linear regression, with the PPPs serving as the dependent variable and the principal components as the independent predictors. This modeling was executed in R, employing the \textit{dplyr}~\citep{wickhamr} and \textit{psych}~\citep{revelle2018procedures} packages. Our validation method comprised five distinct steps:

\begin{enumerate} [topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
\item Conversion of MAST ratings into feature-specific ratings.
\item Implementation of Principal Component Analysis (PCA) to derive principal components from the transformed feature ratings.
\item Identification and selection of the first $k$ principal components responsible for explaining a minimum of 80\% of the total variance, with $k$ being 2 in this study.
\item Application of a linear regression model using the selected principal components as the explanatory variables.
\item Determination of significant principal components (with $\textrm{p-value} \leq 0.05$) and computation of the nested coefficients based on a threshold of 0.3 for the absolute value of PCA factor loadings.
\end{enumerate}

The mathematical representation of the principal component regression utilized in this study is given by:

\begin{equation}
    PPPs = \beta_{1} \cdot PC_1 + \beta_{2} \cdot PC_2 
\end{equation}

where $PC_{i}$ represents the $i^{th}$ principal component, computed as the product of its loadings and the feature ratings ($i={1,2}$), and $\beta_{i}$ denotes the regression coefficients. The expression $\beta_{i} \cdot loadings_{i}$ quantifies the correlation between READIT 2.0's features and the PPPs.

\subsection{PCA Results}

\emily{\autoref{tab:pca} shows the correlation between READIT 2.0's features and the PPPs, illustrating the expected shift in PPP ratings corresponding to a one-standard-deviation increase in the participants' ratings of MAST-informed features.} For instance, an elevation in the rating of the \emph{About Tab} by one standard deviation is predicted to enhance the \emph{purpose} rating by an average of 0.68 units, assuming all other predictors remain constant. This analytical approach enables a nuanced understanding of how specific features influence the overall perception of process, purpose, and performance within the READIT 2.0 framework.

\begin{table}[ht]
\small
\centering
    \begin{tabular}{p{0.35\linewidth}|p{0.15\linewidth}|p{0.13\linewidth}|p{0.13\linewidth}}
      \toprule % <-- Toprule here
      \textbf{Interface Items} & \textbf{Process} & \textbf{Purpose} & \textbf{Performance}\\ 
      \midrule % <-- Midrule here
      \textbf{Data Preprocessing} &  &   \\
      \midrule % <-- Midrule here
      \textbf{Documents Tab} & &  \\
      \midrule % <-- Midrule here
      \textbf{About Tab} &  \textbf{0.477} & \textbf{0.68} & \\    
      \midrule % <-- Midrule here
      \textbf{Topic Clusters} & \textbf{0.287} & \textbf{0.328} & \textbf{0.479} \\
      \midrule % <-- Midrule here
      \textbf{Topic Similarity Matrix} & \textbf{0.314} & \textbf{0.464} & \textbf{0.51} \\                             
      \midrule % <-- Midrule here
      \textbf{Topic Filtering } &  & \textbf{0.412} &\\
      \midrule % <-- Midrule here
      \textbf{Topic Timeline}  &  & \textbf{0.464} & \textbf{0.388}\\
      \midrule % <-- Midrule here
      \textbf{Documents and Summaries} & \textbf{0.246} & \textbf{0.328}  &  \\
      \midrule % <-- Midrule here      
    \bottomrule % <-- Bottomrule here
    \end{tabular}
    \vspace{20pt} \caption{Correlation between READIT 2.0 features and process, purpose, and performance information from trust theory~\citep{lee2004trust}. The values in the table represent the nested coefficients obtained from PCA loadings multiplied by regression coefficients $\beta$. (Detailed information about loadings and coefficients are found here: Appendix \ref{fig:pca} and \ref{fig:lm}.) Blank spaces indicate that certain features do not meet the 0.3 threshold of PCA loadings, suggesting they are not as significant as other features for PPPs.}
  \label{tab:pca}
  % \end{center}
\end{table}


PCA findings reveal that the impact of dominant features on \textit{process}, \textit{purpose}, and \textit{performance} is varied, with multiple features of READIT 2.0 contributing significantly to all three PPP dimensions. Specifically, the \textit{About Tab}, which provides comprehensive descriptions of the technologies underpinning READIT 2.0, alongside \textit{Topic Clusters}, \textit{Topic Similarity Matrix}, and \textit{Documents and Summaries} are associated with \textit{process}. Moreover, the dimension of \textit{purpose} is broadly addressed by all features with the exception of \textit{Data Preprocessing} and \textit{Documents Tab}. The \textit{About Tab} emerges as particularly crucial in this context. This is attributable to the fact that operators seeking detailed insights via the \textit{About Tab} can gain a deeper understanding of READIT 2.0’s functionalities, aligning closely with the informational needs specified by the \textit{purpose} dimension. 

Across the board, the integration of MAST-informed features within READIT 2.0 demonstrates a moderate to strong correlation with the PPPs, indicating their significant influence on the system's trustworthiness. The perception of system \textit{performance} is notably enhanced by the synergistic features of \textit{Topic Clusters}, \textit{Topic Similarity Matrix}, and \textit{Topic Timeline} when a specific topic is selected. \emily{These features together provide a comprehensive and structured understanding of the data through visualization techniques, thereby aiding operators in navigating and using the data more effectively.}

This analysis suggests that adherence to the MAST criteria during the development and selection of features for AI-DSS can substantially foster the calibration of trust by effectively addressing the critical dimensions of \textit{process}, \textit{purpose}, and \textit{performance}. We thus recommend that system designers consider incorporating MAST as part of their design process if a focus of their work is to improve facets of information quality that can affect trust in an AI-DSS. 

% \subsection{Correspondence Analysis}

% \textcolor{blue}{(This subsection including the paragraph and picture below may be not necessary. If the analysis and result above are enough, we can remove this without any harm.)}

% To understand the relationship between features designed via MAST criterion in \textit{READIT 2.0} and Chancey trust theory, we applied correspondence analysis(cite) via summing up all ratings regarding features and building features-PPPs table (without using variables of Chancey trust but based on our discussion and determination). From the biplot of two dimensions in \autoref{fig:ca}, we can see two dimensions cover 100\% variances. Topic Clusters and Topic Similarity Maxtrix have a close relationship with Performance, while Topic Filtering has a strong impact on Purpose. \emph{Data Preprocessing} page and \emph{About} page are relevant features related to Process.  
% %**INCLUDE A LAY-PERSON DESCRIPTION OF OUR EVIDENCE FOR WHY WE THINK THESE FEATURES MAP TO THE THREE Ps**

% \begin{figure}[!ht]
%     \centering
%     \subfloat[\centering All data]{{\includegraphics[width=15cm]{figs/biplot.png}}}
%     \qquad
%     \subfloat[\centering  High MAST]{{\includegraphics[width=15cm]{figs/biplot - high.png}}}
%     \qquad
%     \subfloat[\centering Low MAST]{{\includegraphics[width=15cm]{figs/biplot - low.png}}}
%     \caption{Correspondence Analysis Biplot}
%     \label{fig:ca}
% \end{figure}



==> archive/6discussion.tex <==
\section{Discussion}

To reconcile tradecraft-derived guidelines with a human-centered approach to system design, our methodology \mvm{proposes} MAST as a foundational tool within an interative design process we call PADTHAI-MM. In PADTHAI-MM we use MAST within the stages of goal setting, concept generation, and iterative evaluation. As a case study, PADTHAI-MM outlines the iterative process we followed to develop READIT 2.0, a text summarization system crafted for research purposes and as a medium for evaluating the utility of MAST. \emily{To evaluate MAST, we developed two versions of READIT 2.0: }a High-MAST version, enriched with a comprehensive feature set aimed at augmenting operator task performance, and a Low-MAST version, streamlined to include only the essential features needed for task completion. 

The outcomes of our stakeholder evaluation of READIT 2.0 show significant differences between the High-MAST and Low-MAST versions, both in terms of perceived MAST criteria and trust ratings. Our analysis of the relationship between MAST-informed features and the dimensions of \textit{process}, \textit{purpose}, and \textit{performance} is the first study to demonstrate the trust-theoretic underpinnings of the MAST criteria. Taken together, these results not only validate the practical application of MAST within a design context but also provide evidence for why a MAST-informed design process would support the design and development of more trustable AI-DSS. 

Although beyond the scope of this work, the interrelations among the tradecraft-derived MAST criteria could be clarified through statistical analyses of additional survey data. For instance, a multicollinearity assessment within a regression framework on MAST ratings could identify and mitigate redundancies among MAST features. Understanding MAST criteria synergies might also further benefit from PCA or other analytic techniques like Correspondence Analysis (CA) that could be used to distill MAST criteria into principal components that encapsulate the essence of MAST. This analytic approach would be similar to ~\cite{salehi2023evaluating}, in which a more systematic examination of MAST was conducted.

\subsection{Limitations}
While our case study demonstrates how to use MAST as part of an interactive design process in support of developing more trustable AI-DSS, we acknowledge several limitations of this initial work. First, our findings highlight the perceptual differences between the High-MAST and Low-MAST versions from an operator's perspective. However, higher MAST criteria and trust scores do not necessarily equate to improved task performance outcomes~\citep{salehi2023evaluating}, consistent with the mixed conclusions in the literature on whether trust scores are directly and positively correlated to operational efficiency and effectiveness. Second, the fast-paced evolution of AI technologies and their various application areas may require updates or extensions to the MAST methodology to maintain its long-term relevance and efficacy in the system design and evaluation space. For example, could there be a time when it is more widely recognized that some criteria will be difficult to achieve an ``excellent'' rating on, depending on the criticality (e.g., risk, threat) of the task? What then should technology evaluators do with that information? Third, preliminary analyses indicate potential redundancies among certain MAST criteria within specific task contexts, hinting at opportunities to streamline the framework. Further research should explore the consolidation of criteria to enhance the framework's efficiency without compromising its comprehensiveness. Lastly, navigating the trade-offs between competing MAST criteria, such as the tension between model accuracy and interpretability, remains a challenge. Future endeavors particularly on fielded systems could aim to reconcile these conflicts by considering other impactful design approaches such as~\cite{Roth_Bisantz_Wang_Kim_Hettinger_2021} and potentially merging those approaches with PADTHAI-MM. 

Looking forward, addressing the practical challenges and potential biases in evaluating AI systems is essential for preserving the integrity and effectiveness of MAST as part of a design methodology. We posit that documenting the variability inherent in context-specific ratings of the MAST criteria might highlight areas that require enhanced scrutiny, particularly in defining feature concepts more precisely and operationalizing them in alignment with the rating objectives. For instance, selection bias could occur, which would reduce the benefits of having a multidisciplinary design team. Another challenge lies in the practical evaluation of the criteria, especially in assessing data quality and credibility in real-world cases. Although MAST covers this concern in its \textit{Sourcing} criteria, in READIT 2.0, we modified competition data that had verifiable quality and credibility given the well-scoped task and a known ground truth. However, for more complex AI systems, advanced statistical methods may be required to assess data quality given large corpus data environments where ground truth is virtually unknown \citep{ba2024data}. 
Another approach may involve the integration of adaptive AI architectures and algorithms (e.g., \citealp{madrasPredictResponsiblyImproving2018}) into MAST-inspired system designs to take operator needs and decision biases into consideration when displaying trust-enhancing features or system outputs. As MAST continues to be refined, we encourage future researchers, designers, or developers to consider how different AI models and their application contexts might differ from the ones we discuss here, and to familiarize \emily{themselves }with other design approaches to more comprehensively advance the development of trustable and trustworthy AI systems. 


==> archive/7conclusion.tex <==
\section{Conclusion}
This paper addresses the practical application and theoretical underpinnings of the Multisource AI Scorecard Table (MAST), a tradecraft-derived tool that can be used as a basis for designing AI-enabled decision support systems (AI-DSS). We introduce PADTHAI-MM, a methodology that incorporates MAST as part of an iterative design framework, and details the process of applying this framework in the development of READIT, an AI-DSS research platform for studying human-AI systems.

Building on our previous investigation of MAST~\citep{salehi2023evaluating}; our proposed methodology, case study, and study findings support the value of MAST as a tool for both scholars and practitioners engaged in understanding the facets of information quality that can affect trust in AI-DSS. This work contributes to ongoing efforts to bridge between evaluating for technical reliability and evaluating for people's trust and effective use of these systems. 

